Dynamic Time Warping for Lead-Lag Relationships in Lagged Multi-Factor Models

In multivariate time series systems, lead-lag relationships reveal dependencies between time series when they are shifted in time relative to each other. Uncovering such relationships is valuable in downstream tasks, such as control, forecasting, and clustering. By understanding the temporal dependencies between different time series, one can better comprehend the complex interactions and patterns within the system. We develop a cluster-driven methodology based on dynamic time warping for robust detection of lead-lag relationships in lagged multi-factor models. We establish connections to the multireference alignment problem for both the homogeneous and heterogeneous settings. Since multivariate time series are ubiquitous in a wide range of domains, we demonstrate that our algorithm is able to robustly detect lead-lag relationships in financial markets, which can be subsequently leveraged in trading strategies with significant economic benefits.

==> preamble.tex <==
%load any additional packages

\usepackage[UKenglish]{babel}
\usepackage[utf8]{inputenc} % so we can input characters with accents (e.g. ő)

\usepackage{statsbeamer}

\usepackage{graphicx} % ease graphics management
\graphicspath{{plots/}} % define folder with images
\usefonttheme{serif} % change font to allow \textbf{}
\usepackage{charter} % Nicer fonts

\usepackage{amsmath,amsthm,amssymb} % for math equations

\usepackage{natbib} % richer citation
\usepackage{breakcites} % avoid overfull hbox for long cites
\usepackage{setspace}
\usepackage{multirow}
\usepackage{longtable}
%\usepackage[margin=1.5in]{geometry} 
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{csquotes}
\usepackage{subcaption}
\usepackage{graphicx}
\usepackage{tikz}
\usepackage{lipsum}
\usepackage{tcolorbox}
\usepackage{tabularx}
\usepackage{booktabs}
\usepackage{listings}
\usepackage{titlesec}
\usepackage{biblatex}
